Transferring Procedural Knowledge across Commonsense Tasks

Stories about everyday situations are an essential part of human communication, motivating the need to develop AI agents that can reliably understand these stories. Despite the long list of supervised methods for story completion and procedural understanding, current AI has no mechanisms to automatically track and explain procedures in unseen stories. To bridge this gap, we study the ability of AI models to transfer procedural knowledge to novel narrative tasks in a transparent manner. We design LEAP: a comprehensive framework that integrates state-of-the-art modeling architectures, training regimes, and augmentation strategies based on both natural and synthetic stories. To address the lack of densely annotated training data, we devise a robust automatic labeler based on few-shot prompting to enhance the augmented data. Our experiments with in- and out-of-domain tasks reveal insights into the interplay of different architectures, training regimes, and augmentation strategies. LEAP's labeler has a clear positive impact on out-of-domain datasets, while the resulting dense annotation provides native explainability.

==> section/acknowledgements.tex <==
\section{Acknowledgements}
Yifan Jiang and Filip Ilievski are sponsored by the DARPA MCS program under Contract No. N660011924033 with the United States Office Of Naval Research.

==> section/framework_backup.tex <==

\begin{figure*}[!t]
	\centering
	\includegraphics[width=0.9\textwidth]{img/framework.drawio.pdf}
	\caption{An illustration of Procedural Transfer Framework. The model structure is presented in the green box. The model obtains procedural knowledge from source task TRIP and transfers procedural knowledge through zero-shot evaluation on unseen tasks. Different story models and training regimes are adapted to study their effect on the model's generalizability. Three data augmentation method: participant abstraction, word insertion, and labeling system, is implemented to improve the model's zero-shot performance.}% \filip{Typo: lableing} \yifan{corrected}}
	\label{fig:framework}
\end{figure*}

\section{\method: Procedural Transfer Framework} \label{Framework} 

We design a framework called \method~(Learning from Experience by Annotating Procedures) that enables the transfer of explicit procedural knowledge from a source task $S$ to novel target tasks $T_1, T_2, ...$ in a zero-shot manner. The source task consists of pairs of 
plausible and implausible stories $(P, P^{\prime})$, each consisting of n sentences $s_1,s_2, ... s_n$ and annotated with the following three procedural components: (1) the preconditions and the effects for each attribute $a \in A$ of each participant $e \in E$ at every step in the story; (2) conflicting sentences ($s$,$s^\prime$) pair in the implausible story; and (3) plausibility of the story $P_{plau} \in \{0,1\}$. Ideally, the model that learned procedural knowledge should be able to generalize to unseen tasks that  require similar kinds of reasoning.
Thus, we select target tasks $T_i$ that are 
 in multiple-choice format, where given a partial procedure description, a model has to select the answer that optimally completes the procedure.


% \subsection{Core Modeling Architecture}
The model structure, shown in green in the center of Figure \ref{fig:framework}, is loosely based on CGLI \cite{ma2022coalescing}, which achieves state-of-the-art results on procedural understanding tasks. CGLI takes sentence-participant pair in each story as the procedural text input and combines them with timestamp tokens to mark each step in the text, as input to a Transformer language model. Three distinct output layers are used to perform the stratified reasoning. %\textit{Attribute classifier},\textit{Conflict detector}, and \textit{Story classifier}, use the output from the Transformer model to predict 
%three previous procedural \filip{previous? do you mean following?} \yifan{previous refer to the three objects introduced in the first paragraph."The source task consists of ..."}components. 
\textit{Attribute classifier} predicts the preconditions and the effects for each attribute of each participant. \textit{Conflict detector} predicts the conflict sentences in the story. \textit{Story classifier} determines which story is plausible. 

% Building on this general model, 
Our framework extends this general model with two different story modeling methods, three training regimes and four augmentation strategies. We also evaluate on four out-of-domain tasks (\cref{fig:framework}).

% \filip{please explain here what is the model architecture like in 1 paragraph. The reader should not be expected to know the other paper}
% \yifan{The detail of each model block is introduced in Separate Strategy, including formula and corresponding notation. And we present Joint Strategy by introducing its additional modification compared to the Separate Strategy. Thus, in here, I just simply introduce each block in the model and its function.}


 \subsection{Story Modeling}
% \km{Is the separate strategy the same as CGLI?}
% \yifan{Basically, they are the same, except we use sigmoid when picking the conflict sentence pair.}
%% input representation of different input strategies, introduce separate strategy first and then introduce joint strategy as an addition modification based on former
\method~includes two ways of modeling stories: individually and jointly (as pairs). % a separate story modeling strategy and a joint input strategy based on the model decision pattern. 

\filip{the formalization of this part is good overall, I am just wondering if it becomes a little dense and hard to follow - maybe we can add an example somewhere to help the readability?} \yifan{Maybe we can replace all formulas with plain text and just use formulas or a specific example in input formation and loss training. It is hard for the reader to accept all the complex and detailed ideas in such a short paragraph. Using plain text to introduce at a high level may be better. }

\noindent\textbf{Single Story Model.} 
The method of~\cite{ma2022coalescing} models single stories, i.e., it outputs a plausibility score separately for each story $P$. % in story pairs. \filip{I don't understand the notation in the last sentence}
In this setup, we construct a participant-sentence %\filip{what is entity-first?}\yifan{entity-sentence may be more proper.} 
input representation \cite{gupta-durrett-2019-effective} for each participant at each step of the procedural story. Given an participant $e \in E$, we construct a pseudo question $Q =$ 'where is \{$e$\}' and combine it with n sentences in P, resulting in an input representation $C = [CLS] Q [ SEP] s_1 [SEP] ... s_n [SEP]$. We pass $C$ to a contextual embedding layer to get $C_{emb} \in R^{d\times m}$, where $m$ is the number of tokens and $d$ is the output dimension. Following \cite{rajaby-faghihi-kordjamshidi-2021-time}, we then create a timestamp token (0=padding or pseudo question, 1=past, 2=current, 3=future) for each token in $C_{emb}$, resulting in $T \in R^{m}$, to include step information explicitly. We use another timestamp embedding to get $T_{emb} \in R^{d\times m}$ and pass the sum
%mation \filip{concatenation?} \yifan{We use the summation in our model} 
of $T_{emb}$ and $C_{emb}$ to the Transformer LM to yield $C_{enc} \in R^{d\times m}$. We concatenate $C_{enc}^{i} \in R^{d}$ of each sentence in P and extract the head token $C_{enc}^{N\prime} \in R^{d\times n}$ to represent the global procedural information, which is passed on the attribute classifier, conflict detector, and story classifier.

%% attribute classifier
\textit{Attribute classifier} is a typical two-layer feed-forward classification module that takes $C_{enc}^{i\prime}$ ($i \in n$) in each sentence and predicts corresponding precondition and effect attributes. Given A attributes, we include A precondition classifiers and A effect classifiers. 

%% conflict detector
\textit{Conflict detector} concatenates every pair of \{$C_{enc}^{i\prime}$,$C_{enc}^{j\prime}$\} ($i,j \in n$) and uses a linear layer to find the conflicting pair:
\begin{align}
    & C_{confl} = Stack(Concat(C_{enc}^{i\prime},C_{enc}^{j \prime})) \\
    & P_{confl} = Sigmoid(W_{confl} C_{confl})
\end{align}

\textit{Story classifier} computes mean of all $C_{enc}^{i\prime}$ and use another linear layer for binary classification. Formally:
 \begin{align}
    & C_{plau} = Mean(C_{enc}^{N \prime})\\
    & P_{plau} = Softmax(W_{plau}^T C_{plau})
\end{align}

We use the average of all participants' $P_{confl}$ as the final conflict sentence predictions and use the average of all $P_{plau}$ as the plausible logit of story $P$. We pick the story with the maximum logit value as the plausible story. %\filip{how do you go from compare to pick the story - is it to P plau with a maximum value?} \yifan{add one sentence to explain.}

We jointly optimize over three loss functions corresponding to these classifiers $\textit{L}_{plau}$, $\textit{L}_{confl}$ and $\textit{L}_{attri}$ to train the model with procedural knowledge. $\textit{L}_{attri}$ combines two separate subfunctions: attribute precondition ($\textit{L}_{prec}$) and effect ($\textit{L}_{effe}$). %\filip{I added a sentence to make the losses more readable, pls validate that it makes sense.} \yifan{The new version is great.}

%% Joint input strategy

\noindent\textbf{Joint Story Model.} In discriminative tasks, the model's procedural reasoning may benefit from considering story pairs jointly. Thus,
% As letting the model be aware of the difference in story pairs can enhance the model's understanding of procedural knowledge, 
we newly propose a joint story modeling structure that asks the model to make decisions over pairs of stories. 
%\filip{the motivation in the last sentence is problematic because we don't want a model for TRIP but rather for stories in general. I think we can say that we are 'inspired' by it, or just say that it may happen that two stories have overlapping info.}\yifan{Rephrase the sentence, the tuition of joint story model is letting model learn to compare story pairs and gain knowledge from difference within pairs.} 
Here, we bring additional modifications to input construction and final story prediction. In input construction, for story pair ($P = {s_1,s_2, ...s_n}$,$P^\prime = {s_1^\prime,s_2^\prime, ...s_n^\prime}$) with participant set $E =\{e_1,e_2, ... e_k\}$ in $P$ and $E^\prime =\{e_1^\prime,e_2^\prime, ... e_k^\prime\}$ in $P^\prime$, we first obtain the common participant set $E_c = E\cap E^\prime$. For each common participant $e_{com} \in E_c$, we construct input representation pairs with sentences in each story:
 \begin{align}
    & C = [CLS] Q [ SEP] s_1 [SEP] ... s_n [SEP]\\
    & C^\prime = [CLS] Q [ SEP] s_1^\prime [SEP] ... s_n^\prime [SEP]
\end{align}
where $Q = $ 'where is \{$e_{com}$\}' is same in $C$ and $C^\prime$. For the left unmatched participants $e_{single} \in (E\cup E^\prime -E\cap E^\prime)$, we create pseudo question  $Q_{dummy} =$ 'where is \underline\quad ' with dummy participant \{\underline\quad\} to make up for the missing opposite input representation:
 \begin{align}
    & C = [CLS] Q [ SEP] s_1 [SEP] ... s_n [SEP]\\
    & C^\prime = [CLS] Q_{dummy} [ SEP] s_1^\prime [SEP] ... s_n^\prime [SEP]
\end{align}

Then $C$ and $C^\prime$ go through the same process as the single story modeling with \textit{Attribute classifier} and \textit{Conflict detector} giving the corresponding prediction within each story and \textit{Story classifier} outputting the plausibility score $P_{plau}$ and $P_{plau}^\prime$. In the joint story model, we add an additional \textit{Softmax} layer over $P_{plau}$ and $P_{plau}^\prime$ to pick the more plausible story in each input representation pair.
Finally, we average all story prediction results to get the final prediction.

\subsection{Training Regimes}

As the model optimizes over multiple objectives, we experiment with three training regimes: story-, participant-, and sentence-based. 

%% story based
\noindent\textbf{Story-based loss} optimizes all three losses for each participant input representation:
\begin{equation}
   \textit{L} = \textit{L}_{plau} + \textit{L}_{confl} + \frac{1}{A} \sum_{i=0}^{A} (L_{prec}^{i}+L_{effe}^{i})
\end{equation}
Here we set the story label to implausible for all participants from the implausible story.

%% Entity based

\noindent\textbf{Participant-based loss} modifies the \textit{story-based} loss by setting the story label to implausible only for participant that appear in the conflicting sentences of the implausible story. %\filip{does this mean the entities in the conflicting sentence or something more precise?} \yifan{changed the presentation}

%% Sentence based
\noindent\textbf{Sentence-based loss} omits story loss and only optimizes the attribute and conflict losses:
\begin{equation}
   \textit{L} = \textit{L}_{confl} + \frac{1}{A} \sum_{i=0}^{A} (L_{prec}^{i}+L_{effe}^{i})
\end{equation}
In the final story prediction of \textit{sentence-based loss}, we obtain the negative summation of all $P_{confl}$ and detect which story is more plausible.



%% augmentation
\subsection{Augmentation Strategies}
Procedural text understanding requires accurate participant extraction and rich annotation of their attributes in each step, indicating the laboriousness and challenge of collecting large data. For participant extraction, there is no existing work aiming at picking participants directly from the procedural text. For attribute annotation, previous work \cite{https://doi.org/10.48550/arxiv.2210.10109} focuses heavily on active learning to address this issue, which may bring the noise in new data due to the biased distribution of training data \cite{https://doi.org/10.48550/arxiv.2101.11665}. %\filip{this sentence needs citation for active learning and perhaps one for bias in AL}. \yifan{Added} 
We introduce two approaches for data augmentation: modification of in-domain data and annotation of additional data. 


% introduce three data augmentation strategies, \textit{Automatic Annotation},\textit{Entity Abstraction}, and  \textit{Word Insertion}, to provide a new problem-solving perspective and discuss their effectiveness through comparison. \textit{Automatic Annotation} extract entities and their attribute annotation automatically. \textit{Entity Abstraction} and  \textit{Word Insertion}
 % generate new data from TRIP and inherit attribute annotation from original TRIP directly.

\noindent \textbf{Modification of in-domain data} We experiment with two strategies to modify in-domain data: \textit{Participant Abstraction} and \textit{Word Insertion}, which generate new data from an in-domain corpus and inherit the original attribute annotation directly. % from original TRIP directly. 

The \textit{Participant Abstraction} augmentation is inspired by the work in~\cite{hopner2022leveraging} that replaces specific with generic concepts to aid reinforcement learning. We replace all non-human participants with their direct hypernym in WordNet to generate the new dataset. For example, we replace ``bread" with ``baked goods", and we replace the concept ``pan" with ``cooking utensil". 
The intuition is that a participant's hypernym shares similar physical and pragmatic properties with the original participant, enabling the generated data to reuse the original attribute annotation without bringing the conflict to the whole procedural text.
% \noindent

\textit{Word Insertion}
uses nlpaug \cite{ma2019nlpaug} to add adjectives and adverbs to the existing sentence in the in-domain corpus. Word insertion uses a pretrained language model that gets contextual word embedding %\filip{based on?} \yifan{rephrased}
and updates the original sentence with suitable words. For example, after the word insertion, ``Tom ate the cold soup" may become ``Tom ate the wonderful cold tomato soup". As word insertion merely enriches the participant information, we directly reuse the attribute annotation.

\noindent \textbf{Collection of additional data} The Web contains a vast amount of procedural narratives that can be leveraged as additional data for augmentation. We experiment with two kinds of additional data: \textit{Natural Stories} and \textit{Synthetic Stories}.
In terms of \textit{Natural Stories}, we select ROCStories~\cite{mostafazadeh-etal-2016-corpus}, a real story cloze task dataset centered around daily events. We use \textit{Synthetic Stories} that are automatically generated from the Commonsense Knowledge Graph (CSKG)~\cite{DBLP:journals/corr/abs-2006-06114} based on psychological axioms~\cite{gordon2017formal}. The synthetic collection, whose generation is described in~\cite{ilievski2021story}, includes over 100k plausible commonsense stories based on three story types with corresponding templates: unmet expectations, substitutions, and object modifications. Each plausible story is associated with an implausible story based on minor graph-driven adaptations. For our experiments, we use a stratified sample of three thousand synthetic story pairs.

A key challenge of the additionally collected stories is that they would typically lack the dense annotation assumed by our explainable framework. To bridge this gap, we develop a novel labeling system that can automatically process participant extraction and attribute annotation on any type of data. We describe the labeling system in the next section.


% We adapt our labeling system to do automatic annotation on , an artificial QA set created from KG data as well as 
% The detailed component of the labeling system is demonstrated in Section \ref{labeling}.








